MeKB-Rec: Personal Knowledge Graph Learning for Cross-Domain Recommendation

It is a long-standing challenge in modern recommender systems to effectively make recommendations for new users, namely the cold-start problem. Cross-Domain Recommendation (CDR) has been proposed to address this challenge, but current ways to represent users' interests across systems are still severely limited. We introduce Personal Knowledge Graph (PKG) as a domain-invariant interest representation, and propose a novel CDR paradigm named MeKB-Rec. We first link users and entities in a knowledge base to construct a PKG of users' interests, named MeKB. Then we learn a semantic representation of MeKB for the cross-domain recommendation. To efficiently utilize limited training data in CDR, MeKB-Rec employs Pretrained Language Models to inject world knowledge into understanding users' interests. Beyond most existing systems, our approach builds a semantic mapping across domains which breaks the requirement for in-domain user behaviors, enabling zero-shot recommendations for new users in a low-resource domain. We experiment MeKB-Rec on well-established public CDR datasets, and demonstrate that the new formulation % is more powerful than previous approaches, achieves a new state-of-the-art that significantly improves HR@10 and NDCG@10 metrics over best previous approaches by 24\%--91\%, with a 105\% improvement for HR@10 of zero-shot users with no behavior in the target domain. We deploy MeKB-Rec in WeiXin recommendation scenarios and achieve significant gains in core online metrics. MeKB-Rec is now serving hundreds of millions of users in real-world products.

==> 1-abstract.tex <==
It is a long-standing challenge in modern recommender systems to effectively make recommendations for new users, namely the cold-start problem. Cross-Domain Recommendation (CDR) has been proposed to address this challenge, but current ways to represent users' interests across systems are still severely limited.
We introduce Personal Knowledge Graph (PKG) as a domain-invariant interest representation,
and propose a novel CDR paradigm named MeKB-Rec. 
We first link users and entities in a knowledge base % of interest
to construct a PKG of users' interests, named MeKB.
Then we learn a semantic representation of MeKB for the cross-domain recommendation.
% Then we perform semantic embedding mapping on MeKB for cross-domain recommendation.
% To overcome the insufficiency of training records, MeKB-Rec employs Pretrained Language Models to complement the semantic understanding of MeKB's entities and relations.
To efficiently utilize limited training data in CDR, MeKB-Rec employs Pretrained Language Models 
to inject world knowledge into understanding users' interests.
% to complement the semantic understanding of MeKB's entities and relations.
Beyond most existing systems, our approach builds a semantic mapping across domains which breaks the requirement for in-domain user behaviors, enabling zero-shot recommendations for new users in a low-resource domain.
% We investigate representation learning on MeKB for CDR scenarios, 
We experiment MeKB-Rec on well-established public CDR datasets,
and demonstrate that the new formulation % is more powerful than previous approaches, 
% achieves a new state-of-the-art that nearly doubles HR@10 and NDCG@10 metrics of previous approaches.
achieves a new state-of-the-art that significantly improves HR@10 and NDCG@10 metrics over best previous approaches by 24\%--91\%, with a 105\% improvement for HR@10 of zero-shot users with no behavior in the target domain. 
We deploy MeKB-Rec in WeiXin recommendation scenarios and achieve significant gains in core online metrics. MeKB-Rec is now serving hundreds of millions of users in real-world products.


==> 5-experiments-bak2.tex <==
In this section, we conduct various experiments to compare the recommendation performance of the proposed MeKB-Rec methodology and other CDR baselines. 
We present the detailed experiment settings, results, and analyses.
The goal of the experiments is to answer the following research questions:
\begin{itemize}
    \item \textbf{RQ1}: How does MeKB-Rec perform compared to previous CDR systems?
    \item \textbf{RQ2}: Does MeKB represent a sufficient and accurate description of users' interests?
    \item \textbf{RQ3}: To what extend does the world knowledge in Pretrained Language Models (PLM) in EmbedMe affect recommendation results?
    \item \textbf{RQ4}: Does MeKB-Rec perform better on users with few actions in the target domain?
    % \item \textbf{RQ5}: Is MeKB-Rec a sample-efficient methodology?
    \item \textbf{RQ5}: Does MeKB-Rec improve overall user experience in online recommendation systems?
\end{itemize}


\subsection{Dataset}

We compare MeKB with other baseline methods on two real-world cross-domain recommendation datasets: Amazon \cite{ni2019justifying} and WeChat.


\textbf{Amazon Datasets.} The Amazon dataset is a widely used public recommendation dataset. We selected three popular domains in Amazon: (1) Books, (2) CDs and Vinyl, and (3) Movies and TV, abbreviated as \textbf{Movie, Book and Music}. 
In the CDR problem, we use these three domains of data to construct three cross-domain scenarios. 
Following \citet{cao2022disencdr, liu2020cross}, two domains are combined into one CDR scenario.
We combine the domains into three CDR scenarios: \textbf{Amazon Books $\rightarrow$ Movies}, \textbf{Amazon Books $\rightarrow$ Music}, and \textbf{Amazon Movies $\rightarrow$ Music}. 
The degree of semantic gap between domains in these scenarios are different, which can verify the robustness of methods tested.
Positive interactions are defined as a review score of 4 or above.
Following prior work \cite{cao2022disencdr}, we filter out users and items based on frequency of their interactions. Specifically, we filter out users with less than five positive interactions, and filter out items with <50 positive interactions as the focus of this work is not on cold-start items. We randomly selected 20\% of the overlapped users and placed them in the validation set to verify our effectiveness on the cold-start users. 


% TODO 确认当前划分策略（尤其是zero-shot部分）

\textbf{WeChat Datasets.} We build large-scale CDR datasets extracted from WeChat recommendation scenarios.
% Besides, another dataset used for experimental evaluation is the WeChat dataset.
The dataset comes from real user-item interaction on the WeChat platform, involving three recommendation domains: Articles, Channel (short videos), and Live (live broadcasts).
We set up two cross-domain recommendation scenarios that are \textbf{WeChat Articles $\rightarrow$ Videos} and \textbf{WeChat Videos $\rightarrow$ Live}.
% We sample data from all users' interactions 
and construct CDR datasets with millions of records. 
To construct this dataset, we consider reading an article, fully watching a video, and watching a livestream for $ge>30 seconds$ as positive behaviors. We randomly sample all positives within two months for training and the week after for testing. % TODO 确认几个月？
Similarly, we filter out items with <50 positives. 
% % TODO 等待最终采样策略和数据量级
% In order to compare the recommendation systems comprehensively, we adjusted the distribution balance of items.
% articles, videos and live broadcasts with different popularity. 
Compared with the Amazon dataset, the WeChat dataset covers a much larger scale of users and items.
The detailed parameters of the Amazon and WeChat datasets used in the experiments are show in \autoref{Tab-statis-01}. 
The Overlap Ratio is the fraction of overlapped users of two domains over the number of users in the current domain, i.e. $OR(X,Y) = |U_{X} \cap U_{Y}| / |U_{X}|$.

% defined as the number of users that occur in both source and target domain

\begin{table}[t]
\centering
\caption{Statistics of CDR datasets.}
\label{Tab-statis-01}
\begin{tabular}{lccccc}
\hline
\multicolumn{2}{c}{\textbf{Dataset}}   & Users   & \begin{tabular}[c]{@{}c@{}}Overlap\\ Ratio \end{tabular} & Items  & Records   \\ \hline
\multirow{2}{*}{\textbf{Amazon}} & Books & 163,189   & 4.77 $\%$   & 34,820  & 2,431,128   \\ 
                                 & Movies & 18,386   & 42.33 $\%$   & 24,621  & 707,037   \\ \hline
\multirow{2}{*}{\textbf{Amazon}} & Books  & 163,189   & 4.49 $\%$   & 34,820  & 2,431,128   \\
                                 & Music & 61,229   & 11.97 $\%$   & 24,621  & 707,037   \\ \hline
\multirow{2}{*}{\textbf{Amazon}} & Movies & 18,386   & 42.26 $\%$   & 24,621  & 707,037   \\
                                 & Music & 61,229   & 12.69 $\%$   & 55,219  & 826,490   \\ \hline \hline
\multirow{2}{*}{\textbf{WeChat}} & Articles   & 2,270,800 & 52.19$\%$   & 21,432 & 13,197,438   \\
                                 & Videos & 1,260,491 & 94.02$\%$    & 20,617 & 14,230,730   \\ \hline
\multirow{2}{*}{\textbf{WeChat}} & Videos & 1,308,548 & 55.56$\%$   & 20,617 & 10,275,617   \\
                                 & Live  & 818,773 & 88.79$\%$    & 15,030 & 7,262,557   \\ \hline

\end{tabular}
\end{table}

\textbf{Dataset-specific KG augmentation.}
Although Wikidata is a general KG with rich world information, complementing it with domain-specific knowledge can be helpful for recommendation.
We further incorporate dataset-specific entities into the KG to be considered in building MeKB, to increase item coverage and enrich user representations.
For the Amazon dataset, we include three types of entities available in the dataset: brands, categories, and products, each represented by its textual name. They are considered as additional entities with a lower weight (set to 0.5, 0.3 and 0.1 respectively, where original Wikidata entities are assigned a weight of 1.0)
Entity Linking on these entities are trivial, as each item in the dataset already have these entities denoted.
% TODO what about for WeChat?

% 		■ 文章正例、视频正例、直播正例
% 		■ 文章：100w+级别文章，2-6个月正例，1kw+以上用户（需要至少有一个视频或直播正例），每篇文章带title+content文本，只用阅读正例
% 		■ 视频：100w+级别视频，1-2个月正例，上述1kw的子集；带作者信息和视频的description文本，考虑多样性下采样（完播降采样），可以带一些快滑负例标签
% 			● 尽量在视频domain中不同活跃度都有分布（0正例zero-shot, 1-5 few-shot, 5-10, 11-20, 20-50, 50-100, 100+）
% 		■ 直播：10w+级别主播，1-2个月正例，上述1kw的子集；带主播作者信息和开播描述（不一定用），正负例
% 			● 尽量在直播domain中不同活跃度都有分布（0正例zero-shot, 1-5 few-shot, 5-10, 11-20, 20-50, 50-100, 100+）




% benchmark的其他方法有哪些？

% 比较不同方法（热度、ID、其他方法、我们的方法）、
% 不同人群（0个行为、1-5个行为、5-10个行为，10-50个， 50-100个，100+个）、
% 不同指标（R@10, R@100, MR等）（+排序指标、多样性指标？），
% 证明结论

% TODO: sort datasets with largest-first. also in Table 1.

% Amazon table 1
\begin{table*}[t]
\centering
\caption{Experiments on Amazon CDR Dataset}
\label{Tab-amazon-cdr}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{Books $\rightarrow$ Movies }                 & \multicolumn{2}{c}{Books $\rightarrow$ Music} &   \multicolumn{2}{c}{Movies $\rightarrow$ Music}              \\
\cmidrule(r){2-3} \cmidrule(r){4-5}  \cmidrule(r){6-7}           & HR @ 10  & NDCG @ 10 & HR @ 10 & NDCG @ 10 & HR @ 10 & NDCG @ 10 \\
%\midrule[0.001pt]
\midrule
CMF               & 0.0788 & 0.0292  & 0.0783   & 0.0347    & 0.0733    & 0.0348  \\
CoNet               & 0.0623 & 0.0245  & 0.0647 & 0.0253    & 0.0628    & 0.0246  \\
DCDCSR          & 0.0662 & 0.0301  & 0.0658   & 0.0290    & 0.0661    & 0.0292   \\ 
EMCDR             & \underline{0.0801} & \underline{0.0353}  & \underline{0.0836}   & \underline{0.0393}    & \underline{0.0767}    & \underline{0.0381}  \\
DDTCDR             & 0.0764 & 0.032  & 0.0763   & 0.0322    & {0.0758}    & {0.0316}   \\
SSCDR            & {0.0797} & {0.0346}  & {0.0815}   & {0.0341}    & {0.0754}    & {0.0303}   \\
\midrule
\textbf{MeKB-Rec} & \textbf{0.1128} & \textbf{0.0402}  & \textbf{0.1622}   & \textbf{0.0612}    & \textbf{0.1799}    & \textbf{0.0680}    \\
\bottomrule
\end{tabular}  
\end{table*}



% Amazon table 2 with User frequency
\begin{table*}[t]
\centering
\caption{Frequency-binned analysis on user activity. We split users in the Music test set in the Amazon Books $\rightarrow$ Music scenario, based on their frequency seen in training data, and report HR@10 numbers in each bucket. This analysis measures recommendation performance for users with limited or no behaviors for different approaches.}
\label{Tab-user-frequency}
\begin{tabular}{lcccccccc}
\toprule
\begin{tabular}[c]{@{}c@{}}Action Frequency\\ (\#Users, \#Records) \end{tabular} & \multicolumn{2}{c}{ \begin{tabular}[c]{@{}c@{}}Zero-shot Users: $[0]$\\ (1467, 42339) \end{tabular} }  & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Few-shot Users: $[1, 10)$\\  (16425, 21548) \end{tabular}} &   \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Multi-shot Users: $[10, +\infty)$\\ (11109, 35418) \end{tabular}}  & \multicolumn{2}{c}{ All Users }     \\ 
 \cmidrule(r){2-3} \cmidrule(r){4-5}  \cmidrule(r){6-7} \cmidrule(r){8-9}       & HR@10  & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10  \\
%\midrule[0.001pt]
\midrule
CMF               & 0.0942    & 0.0421  & 0.1033   & 0.0346    & 0.1032    & 0.0352 & 0.0783 & 0.0347  \\
CoNet               & 0.0781    & 0.0404  & 0.0928   & 0.0287    & 0.1001   & 0.0307 & 0.0647 & 0.0253  \\
EMCDR             & \underline{0.0981}    & \underline{0.0533} & \underline{0.1345}   & \underline{0.0615}    & \underline{0.1208}  & \underline{0.0645} & \underline{0.0836} & \underline{0.0393}  \\
DDTCDR             & 0.0863    & 0.0423  & 0.1120   & 0.0554    & 0.1135    & 0.0611 & 0.0763 & 0.0322   \\
\midrule
\textbf{MeKB-Rec} & \textbf{0.3104} & \textbf{0.1130}  & \textbf{0.1623}   & \textbf{0.0731}    & \textbf{0.1268}    & \textbf{0.0368}  & \textbf{0.1622} & \textbf{0.0612} \\
\bottomrule
\end{tabular}  
\end{table*}



\subsection{Experiment Settings}


In the experiments, we randomly divide each dataset into training, validation and test sets according to the ratio of 8:1:1. We also put 20\% overlapped users in test set of target domain for cold-start evaluation. For all experiments, we repeat the training and testing process five times and take the average as the final result.
In terms of evaluation methods, we adopt \textbf{Hit Rate @K} and \textbf{NDCG @K} as the ranking evaluation criteria for the recommendation systems. We sample 1 positive item and 999 negative items to compute the metrics.

For implementation of MeKB-Rec, we distribute totally 1024 samples into 8 A100 GPUs to accelerated training. We adopt $lamb$ with a weight decay of 5e-4 as the optimizer and set its initial learning rate to 5e-4. We train Mekb-Rec for 15 epochs and choose cosine learning rate schedule with first epoch for warm-up. We set batch size to 128, length of sequence to 256 for all experiments.




% TODO: 补充每个baseline的引用
\subsection{Baseline}
We compare our proposed MeKB-Rec method with following state-of-the-art cross-domain recommendation methods:

(1) CMF: Collective Matrix Factorization \cite{singh2008relational-cmf} adopts a Matrix Factorization (MF) method to simultaneously factorize the rating matrices across source and target domains, where user representations are shared between two domains.

% (1) CMF: Collective Matrix Factorization \cite{singh2008relational-cmf} simultaneously factor several metrics to extract multiple relations, and then share parameters among factors when an entity participates in multiple domains.

(2) EMCDR: Embedding-and-Mapping framework for CDR \cite{man2017cross} is proposed for inter-domain recommendation. The method applies both MF and Bayesian Personalized Ranking (BPR) for generating latent factors for users and items. A mapping function with linear and non-linear MLP is used to project representations into a same space for overlapping users in both domains.


% (2) CML: Collaborative Metric Learning focus on the connection between metric learning and collaborative filtering, which learns a joint metric space to encode both users' performance and user-user \& item-item similarity.

(3) SSCDR: Semi-Supervised framework for Cross-Domain Recommendation \cite{kang2019semi-sscdr} is proposed to utilize both overlapping users and source-domain items to train the overlapping function.

% (3) CoNet: Collaborative Cross Networks replaces matrix factorization with neural networks in CDR problem, and builds a cross mapping to connect hidden layers in two base networks.

% (4) NeuMF: Neural Collaborative Filtering for Personalized Ranking replaces the traditional inner product with a neural architecture that can learn an arbitrary function from data.

(4) DDTCDR: Deep Dual Transfer Cross Domain Recommendation \cite{li2020ddtcdr} uses a pretrained autoencoder for user and item initial representation, and constructs a latent orthogonal mapping to extract user features over multiple domains combined with the auto-encoder approach. Users' within-domain preferences and cross-domain preferences are jointly modeled. Note that the auto-encoders are pretrained on recommendation data without incorporating world semantic knowledge.

(5) DisenCDR:  Learning Disentangled Representations for Cross-Domain Recommendation  \cite{cao2022disencdr} is a recent state-of-the-art CDR model that disentangles the domain-shared and domain-specific information through two mutual-information-based disentanglement regularizers, where an information regularizer is used to extract domain-shared representations to encode predictive information for both domains, and an exclusive regularizer encourages domain-specific and domain-shared information to be exclusive.



\subsection{Results}



The evaluation results on Amazon datasets are shown in \autoref{Tab-amazon-cdr}.
% \autoref{Tab-amazon-music-movie} and \autoref{Tab-amazon-book-movie}.
Results on WeChat datasets are in \autoref{Tab-wechat-cdr}.
In all datasets, MeKB-Rec significantly outperforms all other methods by a large margin.

\subsubsection{Amazon Dataset}

In the three cross-domain scenarios of the Amazon experiments, the MeKB method has achieved better recommendation results than other baselines. Specifically, the advantage in the Book \& Video scenario is better than that in the other two scenarios. This result shows that for cross-domain scenarios with large domain gap and less interactive information, the construction of personal interest knowledge graphs has a greater advantage.
On the other hand, the performance of MeKB in the evaluation index of k=10 is more significant than that of k=5, which means that in the process of constructing personal interest KG, the possible points of interest an be expanded, so that the cross-domain recommendation effect is more robust. Some interest points that cannot be transferred directly from source domain can be supplemented by the relationship diffusion of the knowledge graph.




\subsubsection{WeChat Dataset}

% In WeChat experiments, we construct two cross-domain experimental datasets of \textbf{Doc \& Video} and \textbf{Video \& Live} based on real application to compare MeKB\&EmbedMe with other baselines.

On the large-scale WeChat dataset, we compare results between MeKB-Rec and the established YoutubeDNN baseline \cite{youtubednn}.
on both \textit{Articles $\rightarrow$ Videos} and \textit{Videos $\rightarrow$ Live} CDR settings, MeKB-Rec performs significantly better than YoutubeDNN, and the margin of advantage is larger than that of the Amazon dataset.
And for the three cases of $k=10/20/50$, MeKB has achieved better results on most of the indicators, which means that the recommendation effect based on personal interest KG is more in line with the global interest distribution.
An important reason for the difference in the results comes from the fact that there are more interest points and more various entity relationships involved in the real recommendation application.
Table 4 shows the number of entities associated in the Amazon and WeChat datasets. It can be seen that the entities involved in the WeChat is more than ten times that of Amazon, which brings greater challenges to the capabilities of feature capture and migration in the recommendation system.
The change of datasets has amplified the shortcomings of other baseline methods for information extraction and mapping.
Meanwhile, the better performance of MeKB\&EmbedMe also reflects the advantages of knowledge graphs in actual applications.
In fact, the proposed MeKB\&EmbedMe method can be applied to the cross-domain retrieval of WeChat Video and Live domain with full users and items, and it can provide significant information supplements to the recommendation system beyond traditional methods, thereby leading to  the benefits of consumption indicators. 

% Wechat table 1
\begin{table}[t]
\centering
\caption{Experiments on WeChat Dataset}
\label{Tab-wechat-cdr}
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{
\begin{tabular}[c]{@{}c@{}} WeChat\\
    Articles $\rightarrow$ Videos 
\end{tabular}  }  & \multicolumn{2}{c}{
\begin{tabular}[c]{@{}c@{}} WeChat\\
    Video $\rightarrow$ Live
\end{tabular}}  \\
\cmidrule(r){2-3} \cmidrule(r){4-5}     & 
\begin{tabular}[c]{@{}c@{}}  % Video\\
    HR@10 \end{tabular} &
\begin{tabular}[c]{@{}c@{}}  % Video\\
    NDCG@10 \end{tabular}  &
\begin{tabular}[c]{@{}c@{}}  % Live\\
    HR@10 \end{tabular} &
\begin{tabular}[c]{@{}c@{}}  % Live\\
    NDCG@10 \end{tabular}\\
%\midrule[0.001pt]
\midrule
YoutubeDNN         & 0.0225   & 0.0107     & 0.0612 & 0.0305   \\
\textbf{MeKB-Rec}   & \textbf{0.1475}   & \textbf{0.0751}    & \textbf{0.2770}    & \textbf{0.1618}  \\
\midrule
Improved          & \textbf{+555.56\%}   & \textbf{+601.87\%}    & \textbf{+352.61\%}  & \textbf{+430.49\%}   \\
\bottomrule
\end{tabular}  
\end{table}



\subsection{Analysis on MeKB-Rec's Robustness}
The proposed MeKB-Rec uses the personal knowledge graph, MeKB, as a medium for expressing cross-domain interests. This method brings strong robustness reflected in two points:

% TODO(ZS): 这里要再过一下，确保没有无数字支持的论断。这个分析是如何用数字支持的。
% 要看我们最终实际的验证setting。
1) Data utility. Evident from results in \autoref{Tab-amazon-cdr}, MeKB-Rec largely outperforms other methods on all CDR metrics. A key source of the improvement is that MeKB-Rec has a 100\% usage rate of the data in \autoref{Tab-statis-01}, while other methods can only use overlapped users for learning. Our essential advantage is that the original feature representation is not restricted during the MeKB construction step, nor is the user/item in training data required to exist in two domains at the same time. Intuitively, textual features of the items can be mapped to entities of the global knowledge graph via entity linking, providing a stable semantic representation of user interest.

2) Capability of multi-domain fusion. Another advantage of using MeKB as an interest expression medium is that it can integrate interest content from various domains, such as articles, videos and lives treams, into the same representation space. MeKB can also robustly deal with the absence of some modal feature of the users or items. Although the experiments in this paper focus on the scenarios of two domains, the use of MeKB-Rec can be directly adapted to the three or more domains without modification. In practice, we have also used MeKB-Rec to integrate the three-domain features of articles $+$ videos $+$ live broadcasts and migrated to the live broadcast recommendation scene, which has achieved significant improvement.

We noticed that the construction quality of MeKB will be affected by the accuracy of the content understanding model and entity linking method. Specifically, the ambiguity of entity names or the insufficient coverage of entities will cause the representation deviation of MeKB. 
If some future work introduces better models for item entity linking that improves MeKB's expressiveness,
% language and video understanding model or even multi-model, 
MeKB-Rec will achieve a better result.





% wechat线上效果图
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{./Figures/live_exp_fv.pdf}
  \caption{DAU and UCTR relative difference in percentage of MeKB-Rec on the A/B testing of WeChat Live Recommendation. Control group is the production recommendation system and Experiment group is the same system with MeKB-Rec as an additional candidate retrieval method.
  }
  \label{Fig-online-exp}
\end{figure}


% PLM EXP on Amazon
% TODO: only keep movies, not books.
\begin{table*}[t]
\centering
% \caption{Impact of pretrained Language Model. The numbers are tested on different CDR scenarios in the Amazon dataset.}
\caption{Impact of pretrained Language Model in different CDR scenarios on the Amazon dataset.}
\label{Tab-amazon-plm}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Setting} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} \textbf{Scenario 1}\\
    Books $\rightarrow$ Movies  
\end{tabular} }  
& \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} \textbf{Scenario 2}\\
    Books $\rightarrow$ Music  
\end{tabular} }
& \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} \textbf{Scenario 3}\\
    Movies $\rightarrow$ Music  
\end{tabular}} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}   & HR@10  & NDCG@10  & HR@10  & NDCG@10  & HR@10  & NDCG@10 \\
%\midrule[0.001pt]
\midrule
Random   & 0.0510 & 0.0123    & 0.0839 & 0.0295  & 0.0779 & 0.0279  \\
With PLM & 0.1128 & 0.0302   & 0.1622 & 0.0612  & 0.1799 & 0.0680 \\
\midrule
Improved  & \textbf{+121.18\%} & \textbf{+145.53\%}  & \textbf{+93.33\%}  & \textbf{+107.46\%}   & \textbf{+130.93\%}  & \textbf{+143.73\%}   \\
\bottomrule
\end{tabular}
\end{table*}


\subsection{Impact of Pretrained Language Models}

As mentioned above, MeKB has a strong and robust representation capability of users' interest, but this capability also brings the challenge of feature mapping in recommendation. Our proposed MeKB-Rec alleviates the problems of insufficient training records with the help of pretrained language model. In essence, MeKB embodies a large amount of world knowledge contained in the global KG to build a complete expression of users' interests. 
Obviously, the training records in recommendation scenarios cannot cover the semantic information of all entities in the global KG. 
The introduction of the pretrained language model enables the semantic understanding of entities in the global KG by pretraining on massive external corpora.

This hypothesis is confirmed in an ablation study shown in \autoref{Tab-amazon-plm}. We observe a significant decline in recommendation performance in MeKB-Rec, after dropping PLM parameters obtained during pretraining.
The ``w/o PLM parameters'' setting uses the same model architecture, but replaces the parameters with random initialization. 
This indicates that the world semantic knowledge obtained during pretraining is useful for modeling users' interest in the CDR task.
% in recommendation performance after replacing the pretrained language model's parameters
% with random initialization.
% In fact, the EmbedMe algorithm without pretrained language model 
% can only recognize some entities that are more concentrated in the recommendation training records. 
We suggest that future work may try to pretrain the language model by the corpus from the target recommendation domain to improve the adaptation effect to the recommendation system.



\subsection{Frequency-binned Analysis on User Activity}

To understand how well our method performs for users with a limited amount of training data, we split users in the Movies test set based on their frequency seen in training data in the target domain, and report HR@10 numbers in each bucket. As shown in \autoref{Tab-user-frequency},
MeKB-Rec shows a significant advancement especially for zero-shot user group (appearing zero times in the training set) and few-shot users (seen less than ten times in training) compared to other methods. 
MeKB-Rec performs less well on high-activity users with more than 100 training examples, as the baseline methods usually have a dedicated ID embedding that fits these users better after seen many examples. 
MeKB-Rec is better for zero-shot and few-shot users which is a critical challenge in CDR.
% TODO




\subsection{Online Experiments}

We conduct A/B experiments in the WeChat online recommendation system serving hundreds of millions of users. We report results in a major Live-stream recommendation scenario in the platform, where we deploy MeKB-Rec to leverage user behaviors in the short video domain to improve recommendation for live streams, especially for cold-start users.

The control group is the current recommendation system in production. The experiment group is the same system with MeKB-Rec as an additional retrieval step for recommendation candidates.
Experiments are run for 10 days, during which the item tower of MeKB-Rec is continuously trained on an hourly basis, to fit recently-popular live broadcasters. 
We focus on two metrics: (1) DAU of non-active users in Live, and (2) Overall UCTR for all users, which is the unique click-through rate on the user level.

The experimental result is shown in \autoref{Fig-online-exp}. X-axis is the day of the experiment, and Y-axis is the relative percentage improvement of the experiment group compared to the control. 
The metric shown in the DAU chart is accumulative while the UCTR chart shows a daily metric. The error bar stands for 95\% confidence interval.
Overall, the experiment group with MeKB-Rec achieves a significant gain of DAU $+0.531\%$ ($p<0.01$) for non-active users, suggesting strong improvements over cold-start (zero-shot and few-shot) users. This pool of users accounts for a significant proportion, and is critical for the growth of the recommendation scenario. The overall UCTR of all users are improved by $+0.240\%$ ($p<0.01$), indicating that users are generally more in favor of the recommended content compared to the baseline.

As online experiments show significant gains, MeKB-Rec has been deployed to the production system for 100\% of non-active users in this scenario.



% \subsection{Sample Efficiency}

% We further study sample efficiency as shown in \autoref{Figure5}.
% As demonstrated, 
% % MeKB-Rec remains strong performance while we reduce the amount of training data used. 
% MeKB-Rec keeps strong performance while the amount of training data decreases, while performance for some other methods drops sharply when using only partial training data. This demonstrates that MeKB-Rec is a sample-efficient method thanks to the few-shot learning capability of PLM.
% We hypothesize that the efficiency is benefited from the few-shot ability of PLM, i.e. the pretrained model has a strong inductive bias of world semantic knowledge inherently useful for transferring users' interest representations.
% Impressively, MeKB-Rec still exceeds other methods' full performance while using only 25\% of available training data.  % TODO



==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
